PILoRA: Prototype Guided Incremental LoRA for Federated Class-Incremental Learning

Existing federated learning methods have effectively dealt with decentralized learning in scenarios involving data privacy and non-IID data. However, in real-world situations, each client dynamically learns new classes, requiring the global model to classify all seen classes. To effectively mitigate catastrophic forgetting and data heterogeneity under low communication costs, we propose a simple and effective method named PILoRA. On the one hand, we adopt prototype learning to learn better feature representations and leverage the heuristic information between prototypes and class features to design a prototype re-weight module to solve the classifier bias caused by data heterogeneity without retraining the classifier. On the other hand, we view incremental learning as the process of learning distinct task vectors and encoding them within different LoRA parameters. Accordingly, we propose Incremental LoRA to mitigate catastrophic forgetting. Experimental results on standard datasets indicate that our method outperforms the state-of-the-art approaches significantly. More importantly, our method exhibits strong robustness and superiority in different settings and degrees of data heterogeneity. The code is available at \url{https://github.com/Ghy0501/PILoRA}.

==> sec/6_limitation.tex <==
\section{Limitations}
\label{lim}

In our study, we employ the pre-trained Transformer model, renowned for its robust representational capabilities, as the foundational network. Meanwhile, we emphasize the importance of utilizing self-supervised pre-trained weights devoid of class information, thus safeguarding privacy rights. However, from Table~\ref{tab:cifar100_Q},~\ref{tab:cifar100_D} we can observe that there is a gap between the results using self-supervised pre-trained weights and supervised pre-trained weights, and thus we believe that exploring how PEFT methods such as LoRA can improve performance under self-supervised pre-trained weights can be of great help for federated incremental learning tasks.

==> table/ablations.tex <==
\begin{table}[t]
\setlength\tabcolsep{5pt}
\renewcommand\arraystretch{1.1}
\caption{\textbf{Ablation Result (\%) on CIFAR-100}. Experimental results based on self-supervised pre-trained weights. $F_N~(\downarrow)$ is the average forgetting and the calculation process can be referred to~\cite{zhu2021prototype}.}
\label{tab:ablation}
\vskip -0.1in
\centering
\scalebox{0.87}{
\begin{tabular}{c||c c c||c c c} 
\hline
\multicolumn{1}{c||}{Partition} & \multicolumn{3}{c|}{$\alpha=6$} & \multicolumn{3}{c}{$\beta=0.5$} \\ 
\hline
Methods & $A_N$ & Avg. & \multicolumn{1}{c|}{$F_N$.} & $A_N$ & \multicolumn{1}{c}{Avg.} & $F_N$ \\ 
\hline
\multicolumn{1}{c||}{Ours-w/o PR} 
& 26.8 & 30.9 & \multicolumn{1}{c|}{\textbf{5.5}} & 41.4 & 48.8 & \multicolumn{1}{c}{9.3} \\
\multicolumn{1}{c||}{Ours-w/o KD} 
& 54.4 & 76.2 & \multicolumn{1}{c|}{34.2} & 9.8 & 60.9 & \multicolumn{1}{c}{84.3} \\
\multicolumn{1}{c||}{\textbf{Ours}}  
& \textbf{70.7} & \textbf{79.2} & \multicolumn{1}{c|}{8.4} & \textbf{70.4} & \textbf{79.2} & \multicolumn{1}{c}{\textbf{8.6}} \\
\hline
\end{tabular}}
\vskip -0.2in
\end{table}

==> table/cifar100_D.tex <==
\begin{table}[t]
\renewcommand\arraystretch{1.1}
\caption{\textbf{Result (\%) on CIFAR-100}. Result are included for 10 tasks (10 classes per task) and under different degree of \textbf{Distribution-based label imbalance} non-iid setting. The gray part shows the results with self-supervised pre-trained weights.}
\label{tab:cifar100_D}
% \setlength{\tabcolsep}{1.8mm}{
\centering

\begin{tabular}{c||c c||c c||c c} 
\hline
\multicolumn{1}{c||}{Partition} & \multicolumn{2}{c|}{$\beta=0.5$} & \multicolumn{2}{c|}{$\beta=0.1$} & \multicolumn{2}{c}{$\beta=0.05$} \\ 
\hline
Methods & $A_N$ & \multicolumn{1}{c|}{Avg.} & $A_N$ & \multicolumn{1}{c|}{Avg.} & $A_N$ & Avg. \\ 
\hline
\multicolumn{1}{c||}{EWC + FL}  
& 8.7 & \multicolumn{1}{c|}{24.5} & 4.9 & \multicolumn{1}{c|}{13.1} &  4.0 & 11.3 \\
\multicolumn{1}{c||}{LwF + FL}  
& 16.3 & \multicolumn{1}{c|}{35.8} & 7.7 & \multicolumn{1}{c|}{17.8} &  7.7 & 14.9 \\
\multicolumn{1}{c||}{iCaRL + FL}  
& 54.8 & \multicolumn{1}{c|}{63.7} & 48.2 & \multicolumn{1}{c|}{53.5} &  42.9 & 43.8 \\
\multicolumn{1}{c||}{TARGET}  
& 13.3 & \multicolumn{1}{c|}{33.8} & 1.2 & \multicolumn{1}{c|}{13.6} &  4.0 & 12.7 \\
\multicolumn{1}{c||}{L2P + FL}  
& 77.4 & \multicolumn{1}{c|}{83.3} & 71.3 & \multicolumn{1}{c|}{79.4} &  69.4 & 77.0 \\
\multicolumn{1}{c||}{\textbf{Ours}}  
& \textbf{79.3} & \multicolumn{1}{c|}{\textbf{85.9}} & \textbf{78.2} & \multicolumn{1}{c|}{\textbf{84.6}} & \textbf{77.8} & \textbf{84.5} \\
\hdashline
\multicolumn{1}{c||}{L2P + FL}  
& 53.9 & \multicolumn{1}{c|}{51.6} & 62.9 & \multicolumn{1}{c|}{71.4} &  38.7 & 32.2 \\
\multicolumn{1}{c||}{\textbf{Ours}}  
& \textbf{70.4} & \multicolumn{1}{c|}{\textbf{79.2}} & \textbf{69.4} & \multicolumn{1}{c|}{\textbf{78.2}} &  \textbf{67.9} & \textbf{77.8} \\
\hline
\end{tabular}
\end{table}

==> table/cifar100_Q.tex <==
\begin{table}[t]
\renewcommand\arraystretch{1.1}
\caption{\textbf{Result (\%) on CIFAR-100}. Result are included for 10 tasks (10 classes per task) and under different degree of \textbf{Quantity-based label imbalance} non-iid setting. The gray part shows the results with self-supervised pre-trained weights.}
\label{tab:cifar100_Q}
% \setlength{\tabcolsep}{1.8mm}{
\centering

\begin{tabular}{c||c c||c c||c c} 
\hline
\multicolumn{1}{c||}{Partition} & \multicolumn{2}{c|}{$\alpha=6$} & \multicolumn{2}{c|}{$\alpha=4$} & \multicolumn{2}{c}{$\alpha=2$} \\ 
\hline
Methods & $A_N$ & \multicolumn{1}{c|}{Avg.} & $A_N$ & \multicolumn{1}{c|}{Avg.} & $A_N$ & Avg. \\ 
\hline
\multicolumn{1}{c||}{EWC + FL}  
& 5.4 & \multicolumn{1}{c|}{17.8} & 4.7 & \multicolumn{1}{c|}{14.4} &  1.2 & 6.8 \\
\multicolumn{1}{c||}{LwF + FL}  
& 11.4 & \multicolumn{1}{c|}{24.6} & 10.3 & \multicolumn{1}{c|}{19.4} &  3.0 & 9.3 \\
\multicolumn{1}{c||}{iCaRL + FL}  
& 42.2 & \multicolumn{1}{c|}{48.6} & 38.5 & \multicolumn{1}{c|}{42.3} &  26.8 & 28.3 \\
\multicolumn{1}{c||}{TARGET}  
& 6.4 & \multicolumn{1}{c|}{23.9} & 5.7 & \multicolumn{1}{c|}{18.7} &  1.6 & 8.2 \\
\multicolumn{1}{c||}{GLFC}  
& 50.0 & \multicolumn{1}{c|}{66.9} & 50.5 & \multicolumn{1}{c|}{61.0} &  4.4 & 12.5 \\
\multicolumn{1}{c||}{LGA}  
& 62.9 & \multicolumn{1}{c|}{73.5} & 61.4 & \multicolumn{1}{c|}{67.5} &  9.8 & 15.1 \\
\multicolumn{1}{c||}{FedET}  
& 66.0 & \multicolumn{1}{c|}{76.4} & - & \multicolumn{1}{c|}{-} &  - & - \\
\multicolumn{1}{c||}{L2P + FL}  
& 72.8 & \multicolumn{1}{c|}{80.3} & 70.4 & \multicolumn{1}{c|}{79.2} &  63.4 & 72.0 \\
\multicolumn{1}{c||}{\textbf{Ours}}  
& \textbf{79.2} & \multicolumn{1}{c|}{\textbf{85.3}} & \textbf{77.4} & \multicolumn{1}{c|}{\textbf{83.7}} & \textbf{73.2} & \textbf{81.1} \\
\hdashline
\multicolumn{1}{c||}{L2P + FL}  
& 63.4 & \multicolumn{1}{c|}{65.1} & 59.0 & \multicolumn{1}{c|}{58.2} &  2.6 & 5.6 \\
\multicolumn{1}{c||}{\textbf{Ours}}  
& \textbf{70.7} & \multicolumn{1}{c|}{\textbf{79.2}} & \textbf{69.8} & \multicolumn{1}{c|}{\textbf{78.4}} &  \textbf{57.5} & \textbf{68.8} \\
\hline
\end{tabular}
\end{table}

==> table/comm_cost.tex <==
\begin{table}[t]
\setlength\tabcolsep{10pt}
\renewcommand\arraystretch{1.05}
\caption{Comparsion of communication cost per round on CIFAR-100. 10 clients are participated in a round.}
\vskip -0.1in
\label{tab:comm}
\centering
\scalebox{0.87}{
\begin{tabular}{c||c} 
\hline
\multicolumn{1}{c||}{Methods} & \multicolumn{1}{c}{Communication Cost} \\ 
\hline
\multicolumn{1}{c||}{GLFC} & $10.82~\times~10^6$  \\
\multicolumn{1}{c||}{LGA} & $10.82~\times~10^6$  \\
\multicolumn{1}{c||}{TARGET} & $4.64~\times~10^6$  \\
\multicolumn{1}{c||}{FedET} & $1.19~\times~10^6$  \\
\multicolumn{1}{c||}{\textbf{Ours}} & \textbf{$0.77~\times~10^6$}  \\
\hline
\end{tabular}}
\vskip -0.2in
\end{table}

==> table/sup_lora.tex <==
\begin{table}[t]
    \centering
        \caption{Ablation Results (\%) on CIFAR-100. Experimental results based on self-supervised pre-trained weights. $F_N~(\downarrow)$ is the average forgetting and the calculation process can be referred to.}
        \label{tab:ablation}
        \scalebox{1.0}{
        \begin{tabular}{c|| c | c | c | c | c | c | c | c | c | c | c | c} 
        \hline
        \multicolumn{1}{c||}{Block}  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12\\ 
        \hline
        \multicolumn{1}{c||}{$A_N$} & 65.1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12\\ 
        \hline
        \multicolumn{1}{c||}{Avg.} & 74.4 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12\\ 
        \hline
        \end{tabular}}
\end{table}
